Habits of Mind: Reusing Action Sequences for Efficient Planning

When we exercise sequences of actions, their execution becomes more fluent and precise. Here, we consider the possibility that exercised action sequences can also be used to make planning faster and more accurate by focusing expansion of the search tree on paths that have been frequently used in the past, and by reducing deep planning problems to shallow ones via multi-step jumps in the tree. To capture such sequences, we use a flexible Bayesian action chunking mechanism which finds and exploits statistically reliable structure at different scales. This gives rise to shorter or longer routines that can be embedded into a Monte-Carlo tree search planner. We show the benefits of this scheme using a physical construction task patterned after tangrams.

==> old_intro.tex <==
% Discovering the building blocks of a problem is key to its efficient solution. Approaches to problem decomposition are based on extracting patterns from past behavior that delineate subproblems. A class of approaches focuses on past state visitation patterns. \citeA{mcgovern2001automatic} proposed that so-called bottleneck states can be identified at rare state transitions and that they are useful subgoals that link subproblems. Several methods based on the successor representation \cite{machado2017eigenoption, machado2021temporal} use the eigendecomposition of state succession patterns to carve the environment into subproblems. However, these approaches require the agent to have explored the entire state space extensively. This requirement can often not be met in machine learning and robotics. Animals evidently leverage not only patterns in the state space but structure in their previous actions as well. In his \textit{law of exercise}, \cite{thorndike1898animal} described that previously frequent choices are more likely to be repeated, irrespectively of rewards. \cite{gershman2020origin} argues that the law of exercise or, synonymously, perseveration, arises from the trade-off between reward maximization and policy complexity. According to this theory, resource-constrained agents show perseveration if they can save resources by updating their policy less and still achieve reasonable rewards. The theory explains animals' proneness to repeat individual actions.

% However, animals also readily pick up on sequential patterns of action. The action chunking process that underlies skill or habit learning \cite{dhawale2021basal} has also been observed in multi-step decision-making tasks where rats become prone to repeating their actions for all steps in chunks \cite{dezfouli2012habits}. \citeA{dezfouli2013actions} argued that action sequences are not blindly repeated but selected in a goal-directed manner, although their simple task cannot conclusively arbitrate between goal-directed action sequence selection and simpler models.

% \citeA{huys2015interplay} tested how human participants simplified a deep planning problem. They found evidence for three heuristics: fragmentation (breaking up the decision tree into sub-trees), pruning (discarding entire sub-trees with bad starting value), and stochastic memoization. The last of these was reflected in the fact that participants became increasingly prone to repeat frequently used entire paths or subpaths, even though they might not be optimal. In their interpretation, this marks a transfer from flexible but costly computation to the less flexible reliance on past experience. A similar observation was made in a task where participants planned and constructed complex structures that were required to be stable in a virtual environment simulating rigid-body physics \cite{mccarthy2020learning}. During training, participants' construction procedures became increasingly stereotyped.

% It is attractive to leverage temporal patterns in action sequences in order to obtain more lightweight planning algorithms. \citeA{riegler2021embodiment} proposed extending the primitive action repertoire with action chunks. This is inspired by animals' \textit{fixed action patterns} that they perform fast and uninterrupted by state assessment, that is, openloop. However, they bypass the problem of finding the appropriate chunks by simply using all possible combinations of actions, an approach that does not scale due to the exponential growth of the number of chunks as a function of chunk size. 

% We propose a Bayesian sequence model that finds action chunks of appropriate sizes due to this adaptive complexity. We augment Monte-Carlo Tree Search (MCTS) such that the sequence model proposes predictable one-step tree expansions as well as open-loop multi-step expansions. The complexity of the chunks proposed by the HCRP scales with the complexity of the sequences that the agent executed in past episodes, opportunistically saving as much planning cost as possible by reuse. We test our model on a physical construction task called tangram.
